Genetic-tunneling driven energy optimizer for spin systems

A long-standing and difficult problem in, e.g., condensed matter physics is how to find the ground state of a complex many-body system where the potential energy surface has a large number of local minima. Spin systems containing complex and/or topological textures, for example spin spirals or magnetic skyrmions, are prime examples of such systems. We propose here a genetic-tunneling-driven variance-controlled optimization approach, and apply it to two-dimensional magnetic skyrmionic systems. The approach combines a local energy-minimizer backend and a metaheuristic global search frontend. The algorithm is naturally concurrent, resulting in short user execution time. We find that the method performs significantly better than simulated annealing (SA). Specifically, we demonstrate that for the Pd/Fe/Ir(111) system, our method correctly and efficiently identifies the experimentally observed spin spiral, skyrmion lattice and ferromagnetic ground states as a function of external magnetic field. To our knowledge, no other optimization method has until now succeeded in doing this. We envision that our findings will pave the way for evolutionary computing in mapping out phase diagrams for spin systems in general.

==> note.tex <==
% 2022.11.11 讨论纪实

Fig1 
    应该反正introduction 里面 （A）图的色彩如何更加吸引人，DNA有点糊
    (a)与(c)图是否可以结合起来

Fig2
    可选项的优化

Fig3
    是否要突出重点

Fig4

Fig5

Fig6

Fig7

%update baseline
%adaptive baseline

%genetic turnning is prove to be useful in 0K and it will become soft in finiate temp

%Currently, we only support 2D system with at least 400 atoms inside. (4*5)
 %Uppsala Atomistic Spin Dynamics (UppASD) package
